Optimal Completion Distillation for Sequence Learning

We present Optimal Completion Distillation (OCD), a training procedure for optimizing sequence to sequence models based on edit distance. OCD is efficient, has no hyper-parameters of its own, and does not require pretraining or joint optimization with conditional log-likelihood. Given a partial sequence generated by the model, we first identify the set of optimal suffixes that minimize the total edit distance, using an efficient dynamic programming algorithm. Then, for each position of the generated sequence, we use a target distribution that puts equal probability on the first token of all the optimal suffixes. OCD achieves the state-of-the-art performance on end-to-end speech recognition, on both Wall Street Journal and Librispeech datasets, achieving $9.3\%$ WER and $4.5\%$ WER respectively.

==> ocd.tex <==
\section{\acronym: Optimal Completion Distillation}
\mohammad{I am not sure TER works as an operator that takes two operands. Something like $D_{\text{edit}}$ maybe more appropriate?}


\comment{
\begin{figure}[t]
  \centering
    \includegraphics[width=.5\textwidth]{ocd2}
  \caption{Diagram of different RNN cell input and loss strategies in the baseline seq2seq model vs the baseline with schedule sampling and the DOC approach.}
\label{fig:ocd}
\vspace{-0.4cm}
\end{figure}
}

\begin{figure}[t]
\begin{center}
\begin{tabular}{c@{\hspace*{1cm}}c}
      (a) {Teacher Forcing} &
      (b) {Scheduled Sampling} \\[-.1cm]
      \includegraphics[width=0.39\textwidth]{rnn-tf} &
      \includegraphics[width=0.39\textwidth]{rnn-ss} \\
      \includegraphics[width=0.39\textwidth]{rnn-policy} &
      \includegraphics[width=0.39\textwidth]{rnn-ocd} \\[-.1cm]
      (c) {Policy Gradient} &
      (d) {Optimal Completion Distillation}\\
\end{tabular}
\end{center}
\comment{
                \end{tabular}
                \end{figure}
                \begin{figure}[t]
                  \centering
                  \begin{subfigure}[t]{0.5\textwidth}
                      \centering
                      \includegraphics[width=0.75\textwidth]{rnn-tf}
                      \caption{Teacher Forcing}
                      \label{subfig:teacher-forcing}
                  \end{subfigure}%
                  \begin{subfigure}[t]{0.5\textwidth}
                      \centering
                      \includegraphics[width=0.75\textwidth]{rnn-ss}
                      \caption{Scheduled Sampling}
                      \label{subfig:ss}
                  \end{subfigure}
                  \begin{subfigure}[t]{0.5\textwidth}
                      \centering
                      \includegraphics[width=0.75\textwidth]{rnn-policy}
                      \caption{Policy Gradient}
                      \label{subfig:policy}
                  \end{subfigure}%
                  \begin{subfigure}[t]{0.5\textwidth}
                      \centering
                      \includegraphics[width=0.75\textwidth]{rnn-ocd}
                      \caption{Optimal Completion Distillation}
                      \label{subfig:ocd}
                  \end{subfigure}
                  \subref{subfig:teacher-forcing}
}
\label{fig:mle}
\caption{Illustration of different training strategies for autoregressive sequence models:
(a) Teacher Forcing: the model conditions on correct prefixes and is taught to predict the next ground truth token.
(b) Scheduled Sampling: the model conditions on tokens either from ground truth or drawn from the model and is taught to predict the next ground truth token regardless.
(c) Policy Gradient: the model conditions on prefixes drawn from the model and is encouraged to reinforce sequences with a high reward $R(\tilde y)$.
(d) Optimal Completion Distillation: the model conditions on prefixes drawn from the model and is taught to predict an optimal completion policy $\pi^*$ specific to the sampled prefix.
\mohammad{let's have "$\tilde{y}_{t-1}$ or ${y}^*_{t-1}$" and "$\tilde{y}_t$ or ${y}^*_t$" as the inputs to the SS plot}
}
\end{figure}

Let $\bys$ and $\hat{\by}$ denote the target and the predicted output sequences, respectively. The goal is to generate the sequence $\hat{\by}$ one token at a time such that final $\hat{\by}$ is as close as possible to $\bys$. In this setup we propose {\it token edit distance} as the distant metric between $\hat{\by}$ and $\bys$ to optimize {\it token error rate (TER)}. 

As an example of a flaw in teacher forcing the log probability of the correct sequence, consider the target sequence: ``{\it The cat is here.}'' and a character based model has predicted ``{\it A ca}'' as the first $4$ characters. In teacher forcing, the model is trained to predict $y^*_4=$`a' regardless of the model predictions so far. On the other hand, considering the characters generated so far the next token that can lead to the minimum {\it TER} is `t' at time step $4$. 

Inspired by the fact that the next best token is not always the target token at that exact time step conditioned on the generated sequence, we make connections between neural sequence modeling and the Q-learning algorithm from reinforcement learning, where the goal is to estimate the optimal value of each state reward assuming
that one follows the optimal policy from that state forward. The state at each time step $i$ is the generated sequence so far ($\hat{y}_{<i}$) and the context $\bx$. The Q-value is the end reward equal to $-\text{D}(\hat{y},\bys)$ where $D$ is the distance metric.  

\begin{lemma}
\label{th:suffix}
Only concatenating a suffix $r_{j>} = (r_j, r_{j+1}, ... r_T)$ of a reference sequence $r$ can decrease the edit distance between a hypothesis sequence $h$ and the reference sequence. 
\end{lemma}
\begin{proof}

By contradiction, assume there exist a sequence $k$ where $(h\oplus k)$ has smaller edit distance to $r$ than $\forall j: (h\oplus r_{j>})$. Among the non-suffix sequences which result in minimum edit distance choose the sequence $k$ which has maximum shared suffix with $r$. from the end of sequence find the first index $i$ that $k$ differs from $r$.  
If $k_i$ is substituted or deleted in the minimum edit distance matching then replacing $k_i$ with $r_i$ will reduce the edit distance which contradicts with $(h\oplus k)$ having the minimum edit distance. If $k_i$ is matched with an earlier token $r_j, j<i$, then replacing it with $r_i$ will keep the edit distance the same but increases the shared suffix of $k$ with $r$ which contradicts with $k$ having the maximum shared suffix with $r$. Therefore, the sequence $s$ where $(h\oplus s)$ has minimum edit distance with $r$ is always a suffix of $r$.
\end{proof}

In a sequence generation task where the distance metric is {\it TER}, we can calculate the optimal Q-value for all the characters at each state in a highly efficient manner. Based on lemma~\ref{th:suffix} for any prefix sequence $\hat{y}_{<i}$, any sequence $s$ which $\hat{y}_{<i}\oplus s$ results in minimum {\it TER} with target sequence $\bys$ is always a suffix of $\bys$.
Predicting any token other than $s_1$ as the next token ($\hat{y}_i$) results in $\text{\it TER}(\hat{y}_{<i}\oplus s, \bys) + 1$.
Therefore, we only need to find the set of suffixes $\hat{S}_{<i} \equiv \argmin{s\in \text{suffix}(\bys)} \text{\it TER}(\hat{y}_{<i} \oplus s, \bys)$.
 Then,
\begin{equation}
    q[(\hat{y}_{<i},\bx), a]= 
\begin{cases}
    -e^*_{<i},& \text{if } \exists s \in \hat{S}_{<i}: s_1 = a~,\\
    -e^*_{<i}-1,              & \text{otherwise}~,
\end{cases}
\end{equation}
where $e^*_{<i}$ denotes the minimum edit distance value.
Furthermore, for any $j$ and $k$ where $$ \text{\it TER}(\hat{y}_{<i}\oplus y^*_{j>}, \bys) < \text{\it TER}(\hat{y}_{<i}\oplus y^*_{k>}, \bys)~,$$ then $$\text{\it TER}(\hat{y}_{<i},y^*_{<j}) < \text{\it TER}(\hat{y}_{<i},y^*_{<k}).$$
Therefore, in order to find $\hat{S}_{<i}$ we only need to calculate the edit distance of $\hat{y}_{<i}$ with all the prefixes of $\bys$. The prefixes $y^*_{<j}$ which have minimum edit distance with $\hat{y}_{<i}$ correspond with the suffixes $y^*_{>j}$ which minimize  $\text{\it TER}(\hat{y}_{<i}\oplus y^*_{j>}, \bys)$. Therefore, the problem is reduced to calculating the edit distances between all prefixes of $\hat{y}$ and all prefixes of $\bys$ which can be efficiently calculated by dynamic programming in $\mathcal{O}(mn)$, $m$ and $n$ being the length of $\hat{y}$ and $\bys$, respectively. The detailed algorithm is provided in the Supplementary material as well.

Therefore, by Algorithm~\ref{alg:edit} in the sequence prediction task we efficiently compute the optimal policy as the softmax of the Q-values of the teacher. Then we distill \citep{hinton-nips-2014} the optimal completion q-values into the student, the sequence model, by minimizing the Kullback-Leibler (KL)
divergence with temperature $\tau$:
$$ \text{Loss}_\text{KL} = \text{softmax}(q/\tau)\log\frac{\text{softmax}(q/\tau)}{ \pit(\a_i \mid \ba_{<i},\bx)}~,
$$ which since the entropy of $q$ is fixed is equal to the cross entropy between $\text{softmax}(q/\tau)$ and $ \pit(\a_i \mid \ba_{<i},\bx)$. 


\begin{algorithm}
\caption[Caption of Alg]{EditDistanceQ op returns {\bf Q-values} of the tokens at each time step based on the minimum edit distance between a reference sequence $r$ and a hypothesis sequence $h$ of length $t$.
}\label{alg:edit}
\begin{algorithmic}[1]
\Procedure{EditDistanceQ}{${\bf r}$, $\bf h$, $t$}
\State $\forall j \in (1..t)$: $D_{0,j}\gets j $
\State $\forall i \in (1..t)$: $D_{i,0} \gets i$
\For{$i$ in $(1..t)$}
\State minDist $\gets i$
\For{$j$ in $(1..t)$}
\If {$h_i$ = $r_j$}
\State repCost $\gets D_{i-1,j-1}$
\Else
\State repCost $\gets D_{i-1,j-1}+ 1$
\EndIf
\State $D_{i,j} \gets min($repCost, $D_{i-1, j} + 1$, $D_{i, j-1} + 1)$
\If {$D_{i, j} < $ minDist}
\State minDist  $\gets D_{i,j}$
\EndIf
\EndFor
\If{minDist $= i$}
\State $Q_{i, r_1} \gets 1$
\EndIf
\For{$j$ in $(1..t)$}
\If{$D_{i,j} = $ minDist}
\State $Q_{i,r_{j+1}} \gets 1$
\EndIf
\EndFor
\For{all tokens k}
\State $Q_{i,k} \gets Q_{i,k} - 1 - $ minDist
\EndFor
\EndFor
\Return $Q$
\EndProcedure
\end{algorithmic}
\end{algorithm}

